Real3D-Aug: Point Cloud Augmentation by Placing Real Objects with Occlusion Handling for 3D Detection and Segmentation

Object detection and semantic segmentation with the 3D lidar point cloud data require expensive annotation. We propose a data augmentation method that takes advantage of already annotated data multiple times. We propose an augmentation framework that reuses real data, automatically finds suitable placements in the scene to be augmented, and handles occlusions explicitly. Due to the usage of the real data, the scan points of newly inserted objects in augmentation sustain the physical characteristics of the lidar, such as intensity and raydrop. The pipeline proves competitive in training top-performing models for 3D object detection and semantic segmentation. The new augmentation provides a significant performance gain in rare and essential classes, notably 6.65% average precision gain for "Hard" pedestrian class in KITTI object detection or 2.14 mean IoU gain in the SemanticKITTI segmentation challenge over the state of the art.

==> arrow_image.tex <==

% adjust until suit your need.
%\setlength{\arrayrulewidth}{0pt}
%\setlength{\tabcolsep}{10pt}% you can change to a smaller. E.g., 5pt or less.
%\arrayrulecolor{red}
\newenvironment{MyCrazyTable}[6][2cm]%
{%
    \setlength{\arrayrulewidth}{0pt}%
    \setlength{\tabcolsep}{10pt}%
    \newcolumntype{O}[1]%
    {%
        >{%
            \begin{minipage}[c][#1][c]%
            {%
                    ##1\linewidth-2\tabcolsep-1.5\arrayrulewidth%
            }%
            \vspace{\tabcolsep}%
         }%
        c%
        <{%
                \vspace{\tabcolsep}%
                \end{minipage}%
         }%
    }%
    \newcolumntype{I}[1]%
    {%
        >{%
            \begin{minipage}[c][#1][c]%
            {%
                    ##1\linewidth-2\tabcolsep-\arrayrulewidth%
            }%
            \vspace{\tabcolsep}%
         }%
        c%
        <{%
                \vspace{\tabcolsep}%
                \end{minipage}%
         }%
    }%
    \begin{longtable}%
    {%
        |>{\centering}O{#2}%
        |>{\centering}I{#3}%
        |>{\centering}I{#4}%
        |>{\centering}I{#5}%
        |>{\centering}O{#6}%
        |%
    }%
    \hline\ignorespaces%
}%
{%
    \end{longtable}%
    
}

\newcommand{\myrow}{%
\includegraphics[scale=0.45]{graphs/bbox_creation/object_01.png}%
&%
\scalebox{1.1}{$\boldsymbol{\longrightarrow}$}%
&
\includegraphics[scale=0.45]{graphs/bbox_creation/hull_01.png}%
&%
\scalebox{1.1}{$\boldsymbol{\longrightarrow}$}%
&
\includegraphics[scale=0.45]{graphs/bbox_creation/fit_bbox_final.png}%
\tabularnewline\hline%
}



\makeatletter
\newcommand\ratio[2]{%
  \strip@pt\dimexpr#1pt/#2\relax
}
\makeatother 



==> backup_table/backup_table.tex <==


\begin{table*}[t]
%\begin{adjustwidth}{-2.5cm}{}
\centering
\begin{tabular}{lccccccccc} 
\hline
\multirow{2}{*}{$\textbf{Methods}$} & 
\multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
& Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
\hline
\textbf{PointPillar} \\
Baseline           &79.13 &67.09 &65.18 &43.61 &39.87 &37.47 &58.26 &41.66 &39.34\\
Global-Aug    &85.21 &73.14 &67.94 &45.60 &42.62 &40.13 &59.44 &41.71 &39.81\\
Lidar-Aug &\textbf{87.75} &\textbf{77.83} &\textbf{74.90} &59.99 &55.15 &52.66 &-&-&-\\
GT-Aug &80.65 &70.52 &66.50 &49.07 &43.72 &39.64 &70.77 &53.98 &50.37\\
GT-Aug + Global-Aug   &86.28 &76.47 &\bf{73.88} &54.52 &49.04 &45.49 &\bf{77.64} &\bf{61.30} &\bf{58.15}\\
Ped-Ins$_1$              &80.68 &67.52 &66.08 &55.05 &50.76 &47.55 &53.67 &37.37 &35.06\\
Ped-Ins$_1$ + Global-Aug   &84.38 &73.08 &68.11 &\bf{55.72} &51.30 &47.47 &46.33 &33.84 &32.47\\
Cyc-Ins$_1$             &83.21 &67.85 &66.23 &41.79 &38.73 &37.63 &70.79 &50.68 &47.74\\
Cyc-Ins$_1$ + Global-Aug    &84.67 &74.12 &67.97 &46.87 &44.17 &41.77 &72.65 &52.71 &49.04\\
Cyc$_{4.7}$ + Ped$_{6.7}$ + Gl.Aug. &40.37 &40.05 &44.73 &55.50 &\textbf{52.00} &\textbf{49.03} &76.82 &52.74 &50.18\\
Car$_3$ &85.16 &71.88 &66.94 &51.14 &47.43 &45.61 &66.13 &45.96 &43.30\\
Car$_3$ + Global-Aug &84.50 &71.55 &66.66 &49.49 &46.77 &45.18 &64.40 &45.97 &42.74\\

\hline
\hline
\textbf{PV-RCNN} \\
Baseline &87.77 &78.12 &76.88 &58.17 &55.59 &54.30 &76.86 &57.75 &54.89 \\
Global-Aug \\
LiDAR-Aug &90.18 &84.23 &78.95 &65.05 &58.90 &55.52 &-&-&-\\
GT-Aug &88.87 &79.05 &78.39 &65.21 &57.86 &54.27 &86.34 &69.92 &65.39\\
GT-Aug + Global-Aug &89.17 &\textbf{81.92} &\textbf{78.78} &65.69 &59.33 &54.78 &88.30 &\textbf{72.55} &\textbf{67.79}\\
Ped-Ins$_1$ &88.02 &78.32 &77.30 &69.99 &64.74 &59.88 &77.26 &58.33 &57.40\\
Ped-Ins$_1$ + Gl.Aug &89.07 &79.04 &78.37 &70.96 &66.63 &61.14 &78.97 &63.47 &57.31\\
Cyc-Ins$_1$ &88.14 &78.44 &77.47 &63.22 &57.83 &52.68 &82.34 &62.93 &59.37 \\
Cyc-Ins$_1$ + Gl.Aug &89.05 &78.96 &78.32 &65.63 &59.14 &57.47 &82.79 &63.69 &62.39\\
Car$_{??}$ + Cyc$_{4.7}$ + Ped$_{6.7}$ &86.41 &67.63 &67.17 &\textbf{73.57} &\textbf{66.55} &\textbf{62.17} &\textbf{92.69} &65.06 &63.43\\
Car$_{??}$ + Cyc$_{4.7}$ + Ped$_{6.7}$ + Gl.Aug.  &87.02 &68.39 &68.35 &69.13 &64.11 &60.45 &87.05 &67.33 &64.22\\
Car$_3$ &88.70 &78.63 &78.09 &59.12 &56.26 &51.64 &81.83 &58.78 &57.66\\
Car$_3$ + Gl.Aug &\textbf{89.23} &79.11 &78.60 &64.02 &58.81 &57.09 &82.17 &64.23 &58.14\\
\hline
\end{tabular}
\label{tab:results3D}
\caption{Object detection results}
%\end{adjustwidth}
\end{table*}

==> eval_PV_RCNN.tex <==

\newcommand{\tmpcolor}{blue}


\begin{table}
\begin{adjustwidth}{-3.5cm}{}
\centering
\begin{tabular}{lccccccccc} 
\hline
\multirow{2}{*}{$\textbf{Methods - PV-RCNN}$} & 
\multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
& Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
\hline
\textbf{REF} - PV-RCNN &88.86 &78.83& 78.30& 60.56 &53.75 &51.90 &- &- &- \\
\textbf{REF} - PV-RCNN GT-Aug &89.57 &83.90 &78.91 &63.12 &54.84 &51.78 &- &- &- \\
\textbf{REF} - PV-RCNN LiDAR-Aug &90.18 &84.23 &78.95 &65.05 &58.90 &55.52 &- &- &- \\

\hline
\hline

PV-RCNN $_{\text{run 1}}$ &87.51 &78.00 &76.79 &58.39 &55.59 &50.35 &75.91 &56.95 &56.09\\
PV-RCNN $_{\text{run 2}}$ &87.99 &78.25 &77.14 &59.38 &56.66 &51.66 &77.10 &58.47 &57.37\\
PV-RCNN $_{\text{run 3}}$ &87.82 &78.10 &76.71 &56.76 &50.65 &49.34 &77.58 &57.82 &51.21\\
\hline

PV-RCNN GT-AUG $_{\text{run 1}}$ &88.96 &83.33 &78.74 &67.35 &61.12 &56.54 &86.74 &72.95 &68.59\\
PV-RCNN GT-AUG $_{\text{run 2}}$ &89.26 &79.39 &78.83 &63.95 &57.89 &53.36 &87.16 &72.20 &66.72\\
PV-RCNN GT-AUG $_{\text{run 3}}$ &89.30 &83.03 &78.76 &65.77 &58.99 &54.43 &90.99 &72.51 &68.06\\

\hline

PV-RCNN CAR CUTBOX $_{\text{run 1}}$ &84.04 &75.20 &74.84 &53.44 &48.23 &45.34 &63.48 &46.07 &43.79\\ 
PV-RCNN CAR CUTBOX $_{\text{run 2}}$ &88.58 &78.78 &78.17 &57.25 &55.29 &50.59 &76.43 &57.84 &56.94\\
PV-RCNN CAR CUTBOX $_{\text{run 3}}$ &88.37 &78.49 &77.88 &62.94 &57.57 &56.36 &84.58 &58.92 &58.31\\


\hline

PV-RCNN CAR INSERTION $_{\text{run 1}}$ &88.72 &78.69 &78.16 &59.34 &56.40 &51.91 &82.76 &58.63 &57.82\\
PV-RCNN CAR INSERTION $_{\text{run 2}}$ &88.85 &78.62 &78.05 &58.90 &56.18 &51.47 &78.46 &58.80 &57.37 \\
PV-RCNN CAR INSERTION $_{\text{run 3}}$ &88.54 &78.58 &78.05 &59.12 &56.19 &51.53 &84.27 &58.91 &57.78 \\


\hline

PV-RCNN PED INSERTION $_{\text{run 1}}$ &88.39 &78.61 &77.59 &70.69 &66.66 &61.01 &75.86 &57.45 &56.67\\ 
PV-RCNN PED INSERTION $_{\text{run 2}}$ &87.95 &78.21 &77.17 &69.46 &62.19 &59.26 &78.97 &59.37 &57.98\\
PV-RCNN PED INSERTION $_{\text{run 3}}$ &87.73 &78.15 &77.14 &69.82 &65.38 &59.38 &76.94 &58.18 &57.54\\


\hline

PV-RCNN BIKE INSERTION $_{\text{run 1}}$ &88.12 &78.32 &77.46 &63.64 &57.41 &52.44 &80.25 &61.56 &55.41\\ 
PV-RCNN BIKE INSERTION $_{\text{run 2}}$ &88.12 &78.48 &77.39 &65.84 &59.09 &53.72 &83.86 &64.44 &62.50\\
PV-RCNN BIKE INSERTION $_{\text{run 3}}$ &88.19 &78.51 &77.57 &60.19 &56.99 &51.88 &82.90 &62.78 &60.20\\

\hline

CAR Insertion 3 objects $_{\text{run 1}}$ &87.61 &77.19 &77.31 &57.20 &51.68 &50.83 &83.80 &57.87 &56.92\\
CAR Insertion 3 objects $_{\text{run 2}}$ &88.05 &77.13 &77.02 &57.60 &51.39 &50.06 &84.31 &57.92 &57.23\\
CAR Insertion 3 objects $_{\text{run 3}}$ &88.39 &77.63 &77.51 &56.89 &54.06 &50.15 &82.59 &57.54 &56.49\\


\hline

CUSTOM Insertion $_{\text{run 1}}$ &84.79 &67.39 &67.65 &69.74 &63.96 &60.16 &85.91 &65.27 &63.71\\
CUSTOM Ins. $_{\text{1.5x longer train run 1}}$ &84.65 &67.18 &67.51 &70.95 &64.85 &60.68 &90.64 &65.96 &64.42\\
CUSTOM Insertion $_{\text{run 2}}$ &85.53 &67.63 &67.78 &71.05 &65.44 &61.06 &85.06 &66.89 &63.40\\
CUSTOM Insertion $_{\text{run 3}}$ &85.91 & 67.87 &67.97 &69.87 &64.37 &60.57 &86.22 &65.32 &64.10\\


\hline

CUSTOM Ins. NEW $_{\text{run 1}}$ &86.41 &67.63 &67.17 &73.57 &66.55 &62.17 &92.69 &65.06 &63.43\\

\hline

CAR Insertion 3 objects NO COVER$_{\text{run 1}}$ &86.48 &77.33 &76.80 &63.38 &56.57 &51.23 &84.85 &64.85 &58.29\\
CAR Insertion 3 objects NO COVER$_{\text{run 2}}$ &87.53 &77.82 &77.22 \\


\hline 
\\
\hline

\textbf{MASKED} Car - only augmentation &11.72 &9.09 &9.09 &61.86 &55.82 &50.39 &84.03 &57.33 &56.75 \\
\textbf{MASKED} Car - only augmentation ($\frac{1}{2}$ of iters) &9.09 &9.09 &9.09 &59.67 &53.58 &51.94 &71.24 &52.30 &46.47 \\
\textbf{MASKED} Ped - only augmentation &87.92 &78.35 &77.29 &47.69 &42.22 &40.94 &76.92, &63.66 &57.12 \\
\textbf{MASKED} Bikes - only augmentation &88.11 &78.58 &77.51 &59.17 &56.65 &51.70 &80.50 &55.08 &49.27 \\

\hline
\\
\hline
MASKED Car - only aug - test with test aug data &64.62 &63.10 &63.10 &52.74 &51.86 &47.82 &77.38 &57.82 &57.29\\
MASKED Car - only aug - test with train aug data &75.31 &74.48 &74.48 &53.33 &52.62 &48.41 &77.16 &57.71 &57.13\\
\hline




\end{tabular}
\label{default}
\caption{PVRCNN}
\end{adjustwidth}
\end{table}



\textbf{Note 1:} In CAR Insertion 3 objects was intended to add maximally 3 cars. On average were added 2.92 cars per scene. Maximum number of cars were added to approximately 3,475 from 3,711 scenes (93.64\%). To approximately 20 scenes (0.54\%) was not able to add any car.\\

\textbf{Note 2:} In Custom insertion was intended to add 10 cars, 5 cyclist, and 7 pedestrians. On average were added 9.03 cars, 4.7 cyclist, and 6.92 pedestrians per scene. Maximum number of cars were added to approximately 2,785 scenes (75.05\%). Maximum number of cyclists were added to approximately 3,310 scenes (89.19\%). Maximum number of pedestrians were added to approximately 3,647 scenes (98.28\%). To approximately 20 scenes (0.54\%) was not able to add any car. To approximately 55 scenes (1.48\%) was not able to add any cyclists. To approximately 12 scenes (0.32\%) was not able to add any pedestrians.\\

\begin{table}
\begin{adjustwidth}{-1.5cm}{}
\centering
\begin{tabular}{lccccccccc} 
\hline
\multirow{2}{*}{$\textbf{Methods - PointPillar}$} & 
\multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
& Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
\hline
BASELINE 1  &82.32 &67.74 &66.00 &40.76 &37.08 &35.48 &61.15 &42.91 &41.73\\
BASELINE 2  &77.69 &66.77 &65.03 &42.22 &38.39 &36.72 &59.65 &42.72 &40.21\\
BASELINE 3  &77.38 &66.77 &64.50 &47.84 &44.15 &40.21 &53.98 &39.34 &36.07\\
\hline
GT-AUG 1  &84.21 &72.72 &67.46 &42.41 &40.42 &37.45 &55.58 &40.90 &37.43\\
GT-AUG 2  &83.03 &72.52 &67.38 &47.50 &44.08 &40.06 &55.81 &38.66 &36.92\\
GT-AUG 3  &84.84 &73.08 &67.94 &45.36 &43.78 &41.91 &54.40 &39.93 &36.02\\
\hline
GT-AUG 1 /no planes  &86.04 &73.29 &68.05 &46.66 &43.38 &39.92 &62.49 &43.72 &41.86\\
GT-AUG 2 /no planes &84.46 &72.99 &67.90 &45.79 &43.35 &42.22 &59.86 &42.23 &40.42\\
GT-AUG 3 /no planes &85.14 &73.15 &67.86 &44.34 &41.13 &38.24 &55.98 &39.18 &37.14\\
\hline
GT-AUG 1 /w gl. aug. &86.23 &76.34 &73.78 &52.87 &47.53 &44.44 &78.64 &61.84 &59.10\\
GT-AUG 2 /w gl. aug. &86.12 &76.49 &74.35 &55.72 &50.14 &46.14 &77.03 &61.41 &58.34\\
GT-AUG 3 /w gl. aug. &86.49 &76.57 &73.51 &54.98 &49.46 &45.88 &77.24 &60.64 &57.01\\
\hline
PED 1  &82.13 &67.45 &66.04 &54.61 &49.30 &47.59 &55.63 &41.62 &37.91\\
PED 2  &81.79 &67.72 &66.33 &54.88 &51.18 &47.10 &54.22 &36.42 &34.48\\
PED 3  &78.12 &67.40 &65.86 &55.66 &51.81 &47.95 &51.15 &34.07 &32.79\\
\hline
PED 1 /w gl. aug. &84.68 &73.04 &68.10 &54.98 &50.42 &46.90 &48.77 &34.93 &33.54\\
PED 2 /w gl. aug. &84.29 &73.03 &68.14 &57.56 &52.83 &48.83 &43.67 &31.67 &30.08\\
PED 3 /w gl. aug.  &84.18 &73.18 &68.08 &54.62 &50.65 &46.68 &46.56 &34.93 &33.80\\

\hline
BIKE 1  &83.18 &68.15 &66.55 &42.47 &39.07 &38.15 &71.68 &51.37 &47.60\\
BIKE 2  &83.04 &67.71 &66.24 &39.91 &37.20 &36.32 &70.44 &50.42 &48.25\\
BIKE 3  &83.40 &67.70 &65.89 &43.00 &39.93 &38.41 &70.24 &50.24 &47.38\\
\hline
BIKE 1 /w gl. aug.  &85.28 &73.81 &68.16 &47.10 &44.75 &43.49 &75.60 &53.62 &49.78\\
BIKE 2 /w gl. aug.  &84.86 &74.67 &68.14 &46.12 &43.77 &40.89 &70.19 &51.25 &47.29\\
BIKE 3 /w gl. aug.  &83.88 &73.87 &67.62 &47.39 &43.99 &40.92 &72.17 &53.26 &50.05\\
\hline
%\hline
%BASELINE avg  &79.13 &67.09 &65.18 &43.61 &39.87 &37.47 &58.26 &41.66 &39.34\\
%BIKE avg  &83.21 &67.85 &66.23 &41.79 &38.73 &37.63 &70.79 &50.68 &47.74\\
%GT-AUG avg  &86.28 &76.47 &73.88 &54.52 &49.04 &45.49 &77.64 &61.30 &58.15\\
%PED avg  &80.68 &67.52 &66.08 &55.05 &50.76 &47.55 &53.67 &37.37 &35.06\\
\hline
BASELINE avg.           &79.13 &67.09 &65.18 &43.61 &39.87 &37.47 &58.26 &41.66 &39.34\\
GT-AUG avg              &84.03 &72.77 &67.59 &45.09 &42.76 &39.81 &55.26 &39.83 &36.79\\
GT-AUG /no planes avg   &85.21 &73.14 &67.94 &45.60 &42.62 &40.13 &59.44 &41.71 &39.81\\
GT-AUG /w gl. aug. avg  &\bf{86.28} &\bf{76.47} &\bf{73.88} &54.52 &49.04 &45.49 &\bf{77.64} &\bf{61.30} &\bf{58.15}\\
PED avg                 &80.68 &67.52 &66.08 &55.05 &50.76 &\bf{47.55} &53.67 &37.37 &35.06\\
PED /w. gl. aug. avg    &84.38 &73.08 &68.11 &\bf{55.72} &\bf{51.30} &47.47 &46.33 &33.84 &32.47\\
BIKE avg                &83.21 &67.85 &66.23 &41.79 &38.73 &37.63 &70.79 &50.68 &47.74\\
BIKE /w. gl. aug. avg   &84.67 &74.12 &67.97 &46.87 &44.17 &41.77 &72.65 &52.71 &49.04\\


\hline





\end{tabular}
\label{default}
\caption{PointPillar}
\end{adjustwidth}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc}
        \multirow{2}{*}{$\textbf{Distance}$} & 
        \multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
        & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
        \hline
        0-10m :  &81.92 &87.14 &87.90 &74.21 &73.76 &73.08 &86.96 &87.77 &85.77\\
        10-20m :  &89.32 &89.77 &89.33 &54.54 &55.13 &49.62 &84.49 &84.24 &68.46\\
        20-30m :  &81.35 &84.68 &77.75 &36.56 &37.03 &33.07 &75.52 &51.22 &50.78\\
        30-40m :  &41.60 &63.29 &62.17 &5.757 &5.822 &5.797 &32.58 &43.31 &43.31\\
        40-50m :  &0.000 &37.35 &33.46 &0.000 &0.231 &0.305 &0.000 &19.27 &18.68\\
        50-60m :  &0.000 &12.29 &11.14 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        60-70m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        70-80m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        \hline
        \\
        \hline
        0-4m :  &0.000 &0.000 &0.000 &0.000 &0.000 &9.090 &0.000 &0.000 &0.000\\
        4-8m :  &79.31 &86.72 &94.86 &72.97 &65.21 &64.98 &33.83 &51.12 &66.12\\
        8-12m :  &87.48 &88.69 &88.72 &71.00 &71.32 &64.57 &88.06 &87.82 &79.12\\
        12-16m :  &88.97 &89.62 &89.13 &56.27 &56.48 &50.22 &75.04 &75.75 &66.93\\
        16-20m :  &87.43 &88.49 &87.41 &53.00 &53.09 &47.61 &83.50 &82.95 &67.03
    \end{tabular}
    \caption{Distance eval of baseline run 1}
    \label{tab:my_label}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc}
        \multirow{2}{*}{$\textbf{Distance}$} & 
        \multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
        & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
        \hline
        0-10m :  &79.96 &88.75 &89.13 &85.82 &84.00 &77.91 &87.97 &89.12 &80.27\\
        10-20m :  &89.34 &89.76 &89.27 &68.49 &68.23 &61.37 &83.94 &82.96 &74.64\\
        20-30m :  &83.29 &85.73 &78.00 &47.27 &47.74 &45.45 &82.56 &58.06 &58.06\\
        30-40m :  &46.65 &69.15 &63.71 &6.441 &8.192 &7.575 &28.16 &49.19 &48.84\\
        40-50m :  &0.000 &40.61 &38.93 &0.000 &0.279 &0.373 &0.000 &24.13 &23.93\\
        50-60m :  &0.000 &9.740 &8.087 &0.000 &0.000 &9.090 &0.000 &9.090 &9.090\\
        60-70m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        70-80m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        \hline
        \\
        \hline
        0-4m :  &0.000 &0.000 &0.000 &0.000 &0.000 &9.090 &0.000 &0.000 &0.000\\
        4-8m :  &89.80 &94.52 &96.07 &85.03 &77.85 &77.35 &35.15 &53.30 &62.58\\
        8-12m :  &89.45 &89.91 &89.92 &80.99 &75.69 &73.63 &89.27 &89.33 &80.28\\
        12-16m :  &88.21 &88.86 &88.36 &74.82 &69.41 &62.36 &78.56 &78.43 &76.75\\
        16-20m :  &87.67 &88.61 &87.65 &65.44 &67.44 &59.08 &81.17 &79.93 &65.18
    \end{tabular}
    \caption{Distance eval of Ped insertion run 1}
    \label{tab:my_label}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc}
        \multirow{2}{*}{$\textbf{Distance}$} & 
        \multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
        & \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 
        & Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
        \hline
        0-10m :  &83.30 &88.06 &88.60 &85.47 &77.98 &77.60 &90.90 &97.40 &88.66\\
        10-20m :  &89.01 &89.48 &89.08 &57.13 &57.48 &52.23 &90.73 &91.35 &76.31\\
        20-30m :  &83.92 &85.90 &77.86 &48.46 &45.46 &42.63 &81.76 &57.74 &56.89\\
        30-40m :  &45.20 &68.47 &63.49 &8.151 &9.598 &7.994 &33.79 &54.16 &53.95\\
        40-50m :  &0.000 &40.15 &37.82 &0.000 &0.171 &0.171 &0.000 &27.38 &25.89\\
        50-60m :  &0.000 &12.57 &12.57 &0.000 &2.020 &2.020 &0.000 &3.030 &3.030\\
        60-70m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        70-80m :  &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000 &0.000\\
        \hline
        \\
        \hline
        0-4m :  &0.000 &0.000 &0.000 &0.000 &0.000 &3.636 &0.000 &0.000 &0.000\\
        4-8m :  &84.32 &88.04 &88.80 &85.17 &77.59 &77.07 &35.79 &53.75 &69.72\\
        8-12m :  &88.55 &89.25 &89.23 &75.52 &74.49 &67.55 &96.46 &96.44 &87.23\\
        12-16m :  &88.42 &89.08 &88.69 &62.39 &57.36 &51.71 &90.84 &92.15 &76.25\\
        16-20m :  &87.41 &88.26 &87.59 &52.90 &56.06 &50.75 &84.38 &83.36 &73.63
    \end{tabular}
    \caption{Distance eval of Bike insertion run 2}
    \label{tab:my_label}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{graphs/add_car_distance.png}
    \caption{Distance of cars in car insertion}
    \label{fig:car_insertion_distance}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{graphs/add_car_occlusion.png}
    \caption{Caption}
    \label{fig:car_insertion_occlusion}
\end{figure}



\begin{table}
\begin{adjustwidth}{-3.5cm}{}
\centering
\begin{tabular}{lccccccccc} 
\hline
\multirow{2}{*}{$\textbf{Methods}$} & 
\multicolumn{3}{c}{$\textbf{AP}_{\text{Car}}$ \textbf{70}($\%$)}
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Ped}}$ \textbf{50}($\%$)}  
& \multicolumn{3}{c}{$\textbf{AP}_{\text{Cyc}}$ \textbf{50}($\%$)} \\ 

& Easy & Mod & Hard & Easy & Mod & Hard & Easy & Mod & Hard\\
\hline

\textbf{REF} - PV-RCNN &88.86 &78.83& 78.30& 60.56 &53.75 &51.90 &- &- &- \\
\textbf{REF} - PV-RCNN GT-Aug &89.57 &83.90 &78.91 &63.12 &54.84 &51.78 &- &- &- \\
& \color{\tmpcolor}+0.71 & \color{\tmpcolor}+5.07 &\color{\tmpcolor}+0.61&\color{\tmpcolor}+2.56&\color{\tmpcolor}+1.09&\color{red}-0.12&-&-&-\\
\textbf{REF} - PV-RCNN LiDAR-Aug &90.18 &84.23 &78.95 &65.05 &58.90 &55.52 &- &- &- \\
&\color{\tmpcolor}+1.32&\color{\tmpcolor}+5.4&\color{\tmpcolor}+0.65&\color{\tmpcolor}+4.49&\color{\tmpcolor}+5.25&\color{\tmpcolor}+3.62&-&-&-\\

\hline
\hline

PV-RCNN BASELINE &87.77 &78.12 &76.88 &58.17 &55.59 &54.30 &76.86 &57.75 &54.89\\
\hline

PV-RCNN GT-AUG &89.17 &81.92 &78.78 &65.69 &59.33 &54.78 &88.30 &72.55 &67.79\\
&\color{\tmpcolor}+1.40&\color{\tmpcolor}+3.80&\color{\tmpcolor}+1.90&\color{\tmpcolor}+7.52&\color{\tmpcolor}+3.74&{\color{\tmpcolor}+0.48}&\color{\tmpcolor}+11.44&\color{\tmpcolor}+14.80&\color{\tmpcolor}+12.90\\


\hline

PV-RCNN CAR INSERTION &88.70 &78.63 &78.09 &59.12 &56.26 &51.64 &81.83 &58.78 &57.66 \\
&\color{\tmpcolor}+0.93&\color{\tmpcolor}+0.51&\color{\tmpcolor}+1.21&\color{\tmpcolor}+0.95&\color{\tmpcolor}+0.67&\color{red}-2.66&\color{\tmpcolor}+4.97&\color{\tmpcolor}+1.03&\color{\tmpcolor}+2.77\\


\hline

PV-RCNN PED INSERTION &88.02 &78.32 &77.30 &69.99 &64.74 &59.88 &77.26 &58.33 &57.40\\ 
&\color{\tmpcolor}+0.25&\color{\tmpcolor}+0.20&\color{\tmpcolor}+0.42&\color{\tmpcolor}+11.82&\color{\tmpcolor}+9.15&\color{\tmpcolor}+5.58&\color{\tmpcolor}+0.40&\color{\tmpcolor}+0.58&\color{\tmpcolor}+2.51\\


\hline

PV-RCNN BIKE INSERTION &88.14 &78.44 &77.47 &63.22 &57.83 &52.68 &82.34 &62.93 &59.37\\ 
&\color{\tmpcolor}+0.37&\color{\tmpcolor}+0.32&\color{\tmpcolor}+0.59&\color{\tmpcolor}+5.05&\color{\tmpcolor}+2.24&\color{red}-1.62&\color{\tmpcolor}+5.48&\color{\tmpcolor}+5.18&\color{\tmpcolor}+4.48\\

\hline

CAR Insertion 3 objects &88.02 &77.32 &77.28 &57.23 &52.73 &50.35 &83.57 &57.78 &56.88\\ 
&\color{\tmpcolor}+0.25&\color{red}-0.80&\color{\tmpcolor}+0.40&\color{red}-0.94&\color{red}-2.86&\color{red}-3.95&\color{\tmpcolor}+6.71&\color{\tmpcolor}+0.03&\color{\tmpcolor}+1.99\\

\hline

CUSTOM Insertion &85.41 &67.63 &67.80 &70.22 &64.59 &60.60 &85.73 &65.83 &63.74\\ 
&\color{red}-2.36&\color{red}-10.49&\color{red}-9.08&\color{\tmpcolor}+12.05&\color{\tmpcolor}+9.00&\color{\tmpcolor}+6.30&\color{\tmpcolor}+8.87&\color{\tmpcolor}+8.08&\color{\tmpcolor}+8.85\\

\hline

CUSTOM Ins. $_{\text{1.5x longer train run 1}}$ &84.65 &67.18 &67.51 &70.95 &64.85 &60.68 &90.64 &65.96 &64.42\\
&\color{red}-3.12&\color{red}-10.94&\color{red}-9.37&\color{\tmpcolor}+12.78&\color{\tmpcolor}+9.26&\color{\tmpcolor}+6.38&\color{\tmpcolor}+13.78&\color{\tmpcolor}+8.21&\color{\tmpcolor}+9.53\\

\hline

CUSTOM Ins. NEW $_{\text{run 1}}$ &86.41 &67.63 &67.17 &73.57 &66.55 &62.17 &92.69 &65.06 &63.43\\
&\color{red}-1.36&\color{red}-10.49&\color{red}-9.71&\color{\tmpcolor}+15.40&\color{\tmpcolor}+10.96&\color{\tmpcolor}+7.87&\color{\tmpcolor}+15.83&\color{\tmpcolor}+7.31&\color{\tmpcolor}+8.54\\

\hline


\end{tabular}
\label{default}
\caption{Average result}
\end{adjustwidth}
\end{table}


%\colorbox{green}{-} 
%PV-RCNN PED INSERTION$_{\text{run 1}}$ &87.86 &78.22 &77.43 &39.83 &37.83 &34.05\\ 
%PV-RCNN PED INSERTION$_{\text{run 2}}$ &87.82 &78.21 &77.23 &46.79 &41.67 &40.69\\
%PV-RCNN PED INSERTION$_{\text{run 3}}$ &88.33 &78.34 &77.41 &36.69 &31.78 &32.07\\


==> predictions.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|r|r|r|r|r|}\hline
         &  TP & FP & FN & Precision[\%] & Recall[\%]\\\hline
    Baseline easy& 2660 & 1940 & 183& -& -\\\hline
    Baseline moderated& 6583 & 4324 & 1189& -& -\\\hline
    Baseline hard& 8811 & 4324 & 2044& -& -\\\hline
    Baseline total& 18060 & 10588 & 3416& 63.04& 84.09\\\hline
    Car insertion easy& 241 & 597 & 2662& -&-\\\hline
    Car insertion moderated& 341 & 1121 & 7534& -&-\\\hline
    Car insertion hard& 394 & 1121 & 10567& -&-\\\hline
    Car insertion total& 976 & 2839 & 20763& 25.58&4.7\\\hline
    \end{tabular}
    \caption{Number of true positive (TP), false positive (FP), and false negative (FN) predictions.}
    \label{tab:TP_FP_FN_predictions}
\end{table}
\textbf{Note 3:} Car insertion model was learned just on inserted cars without original annotations.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{graphs/test_dataset/annotated_car_position.png}
    \caption{Positions of ground truth annotations}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
\hspace*{-2cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-4cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/3 cars insertion without cover/prediction_TP_car_position.png}
    \caption{Car insertion}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \hspace*{5cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-3cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/baseline/prediction_TP_car_position.png}
    \caption{Baseline}
    \label{fig:f2}
  \end{subfigure}
  \caption{Positions of true positive Cars predictions on test dataset}
\end{figure}

\begin{figure}[]
\hspace*{-2cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-4cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/3 cars insertion without cover/prediction_FP_car_position.png}
    \caption{Car insertion}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \hspace*{5cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-3cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/baseline/prediction_FP_car_position.png}
    \caption{Baseline}
    \label{fig:f2}
  \end{subfigure}
  \caption{Positions of false positive Cars predictions on test dataset}
\end{figure}

\begin{figure}[]
\hspace*{-2cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-4cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/3 cars insertion without cover/prediction_FN_car_position.png}
    \caption{Car insertion}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \hspace*{5cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-3cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/baseline/prediction_FN_car_position.png}
    \caption{Baseline}
    \label{fig:f2}
  \end{subfigure}
  \caption{Positions of false negative Cars predictions on test dataset}
\end{figure}

\begin{figure}[]
\hspace*{-2cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-4cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/3 cars insertion without cover/maximal_confidence.png}
    \caption{Car insertion}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \hspace*{5cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-3cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/baseline/maximal_confidence.png}
    \caption{Baseline}
    \label{fig:f2}
  \end{subfigure}
  \caption{Maximal confidence of Cars predictions on test dataset}
\end{figure}

\begin{figure}[]
\hspace*{-2cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-4cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/3 cars insertion without cover/average_confidence.png}
    \caption{Car insertion}
    \label{fig:f1}
  \end{subfigure}
  \hfill
  \hspace*{5cm}
  \begin{subfigure}[b]{0.4\textwidth}
  \hspace*{-3cm}
    \includegraphics[width=2.5\textwidth]{graphs/test_dataset/baseline/average_confidence.png}
    \caption{Baseline}
    \label{fig:f2}
  \end{subfigure}
  \caption{Average confidence of Cars predictions on test dataset}
\end{figure}
